Dynamical gluon effects in the three-dimensional structure of pion

We investigate the internal structure of the pion, including the contributions from one dynamical gluon, using the basis light-front quantization (BLFQ) approach. By solving a light-front QCD Hamiltonian with a three-dimensional confining potential, we obtain the light-front wavefunctions (LFWFs) for both the quark-antiquark and quark-antiquark-gluon Fock sectors. These wavefunctions are then employed to compute the unpolarized generalized parton distributions (GPDs) and the transverse-momentum-dependent parton distributions (TMDs) of valence quarks and gluons. We also extract the transverse spatial distributions, providing the squared radii of quark and gluon densities in the impact-parameter space. This work contributes toward a three-dimensional understanding of the pion's internal structure in both momentum and coordinate space.

==> preamble_math_physics.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% 1.math mode general functionalities %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsmath,amssymb,mathtools} 
    %CCC ams math, ams symbol and math tools
\ifpdftex
    % \usepackage[notext]{stix2}
    \usepackage{bbm}
    \newcommand{\mybb}[1]{\mathbbm{#1}}
    \newcommand{\mybf}[1]{\boldsymbol{#1}}
    \newcommand{\mycal}[1]{\mathcal{#1}}
\else
    \usepackage[bold-style=ISO]{unicode-math}
        %CCC unicode-math for a better scheme to change the math font and also to render different style like \symbf \symbb \symit et al. But, if one only need to get an italic boldface then one could simply use \usepackage{bm}, \pmb{p}, \boldsymbol{p}. If one just want to extend the original \mathbb command to, for example, correctly showing blackboard style number, one may just use \usepackage{bbm}, \usepackage{stix2}. A list of useable math font can be found on: https://tug.org/pracjourn/2006-1/hartke/hartke.pdf and https://tex.stackexchange.com/a/30066/239820
        \setmathfont{latinmodern-math.otf}
        \setmathfont[range=bb]{TeX Gyre DejaVu Math}
        \newcommand{\mybb}[1]{\symbb{#1}}
        \newcommand{\mybf}[1]{\symbf{#1}}
        \newcommand{\mycal}[1]{\symcal{#1}}
\fi



\usepackage{siunitx}  
    %CCC basically provide those three powerful macro \num, \ang, \si to express physical number with unit properly.
    \sisetup{detect-all = true}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% 2.math-related %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% 2.a.general purpose %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


    %CCC to produce delimiter of arbitrary size. usage: \vast{2}|
\makeatletter
\newcommand{\vast}[1]{\bBigg@{#1}}
\makeatother
    
\newcommand{\abs}[1]{\left|#1\right|}

\newcommand{\queseq}{\pmb{\quesclr \stackrel{\mbox{?}}{=}\color{black}}}
\newcommand{\intd}[3][]{\ifthenelse{\isempty{#3}}{\mathrm{d}^{#1} #2}{\frac{\mathrm{d}^{#1} #2}{#3}}\;}
\newcommand{\rmd}{\mathrm{d}}


    %CCC long equal sign with text above it. the equal sign will not extend according to the length of the text
\newcommand{\eqtext}[1]{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\small\rmfamily #1}}}{=}}}
\newcommand{\Leqtext}[1]{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\small\rmfamily #1}}}{=\mathrel{\mkern-3mu}=}}}
\newcommand{\LLeqtext}[1]{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\small\rmfamily #1}}}{=\mathrel{\mkern-3mu}=\mathrel{\mkern-3mu}=}}}
\usepackage{stackengine}
\newcommand{\stackequal}[2]{%
    \mathrel{\stackunder[2pt]{\stackon[4pt]{=\mathrel{\mkern-3mu}=\mathrel{\mkern-3mu}=}{$\scriptscriptstyle#1$}}{%
    $\scriptscriptstyle#2$}}}

\newcommand{\mydprime}{\prime\prime}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  2.b.logic and set theory     %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\Exists}{\exists}
\DeclareMathOperator{\Forall}{\forall}
\newcommand{\Logiceq}{\Longleftrightarrow}
\newcommand{\logiceq}{\Leftrightarrow}
\newcommand{\logicand}{\; \&\& \;}
\newcommand{\Tiff}{{\itshape iff}}
\newcommand{\sucht}{\,{}:\,}
\newcommand{\cond}{\; | \;}
\newcommand{\setcond}[2]{\ifthenelse{\isempty{#2}}{\{#1\}}{\{#1\cond{}#2\}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  2.c.topological and metric space  %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\interior}[1]{\mathrm{int}\,{}#1}
\newcommand{\clos}[1]{#1^{-}}
\newcommand{\bound}[1]{\partial #1}
\newcommand{\diam}[1]{\mathrm{diam}\,{}#1}
\newcommand{\supm}[1]{\mathrm{sup}\,{}#1}
\newcommand{\infm}[1]{\mathrm{inf}\,{}#1}
\newcommand{\homot}{\simeq}
\newcommand{\pathhmt}{\sim}
\newcommand{\pathprod}{\cdot}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  2.d.matrix  %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \newcommand{\tr}{\mathrm{Tr}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% 3.physics-related %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% 3.a. general physics  %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{physics}
    %CCC braket command is more user friendly in this package than in the \usepckage{braket} with automatic sizing
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% 3.b.general high energy physics  %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{braket}
\usepackage{cancel}
    %CCC This package provide \cancel{} to draw crossline in its argument. I think that \cancel is better to look than \slashed
    \def\slashed#1{\cancel{#1}}
        %CCC this is for compatibility purpose

\newcommand{\norord}[1]{\mathbf{:}\mathbin{#1}\mathbf{:}}
\newcommand{\Tord}[1]{T\left(#1\right)}
\newcommand{\gev}[1]{{#1\,\mathrm{GeV}}}
\newcommand{\gevSq}[1]{{#1\,\mathrm{GeV}^2}}
\newcommand{\mev}[1]{{#1\,\mathrm{MeV}}}
\newcommand{\mevSq}[1]{{#1\,\mathrm{MeV}^2}}


\newcommand{\FUU}{F_{UU}}
\newcommand{\FUUphi}{F_{UU}^{\cos\phi}}
\newcommand{\FUUIIphi}{F_{UU}^{\cos2\phi}}
\newcommand{\AUThminusS}{A_{UT}^{\sin\left(\phi_h-\phi_S\right)}}
\newcommand{\AUTIIIhminusS}{A_{UT}^{\sin\left(3\phi_h-\phi_S\right)}}
\newcommand{\AUThplusS}{A_{UT}^{\sin\left(\phi_h+\phi_S\right)}}
\newcommand{\ALThS}{A_{LT}^{\cos\left(\phi_h-\phi_S\right)}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%  3.c.BLFQ  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\LCm}{{-}} 
\newcommand{\LCp}{{+}}
\newcommand{\LCpm}{{\pm}}
\newcommand{\LCmp}{{\mp}}
\newcommand{\LCperp}{{\perp}}
\newcommand{\LCperpinner}[2]{#1^{\perp} #2^{\perp}}
\newcommand{\LCinner}[2]{\frac{1}{2}#1^{+} \cdot #2^{-}+\frac{1}{2}#1^{-} \cdot #2^{+}-#1^{\perp} \cdot #2^{\perp}}

\newcommand{\nmax}{N_{\mathrm{max}}}
\newcommand{\perpSq}[1]{(#1^{\perp})^2}
\newcommand{\perpAbs}[1]{|#1^{\perp}|}
\let\ppSq\perpSq
\let\ppAbs\perpAbs

\newcommand{\fI}[1]{f_1^{#1}}
\newcommand{\fITperp}[1]{f_{1T}^{\perp #1}}
\newcommand{\gI}[1]{g_{1}^{#1}}
\newcommand{\gIL}[1]{g_{1L}^{#1}}
\newcommand{\gIT}[1]{g_{1T}^{#1}}
\newcommand{\hI}[1]{h_{1}^{#1}}
\newcommand{\hIT}[1]{h_{1T}^{#1}}
\newcommand{\hITperp}[1]{h_{1T}^{\perp #1}}
\newcommand{\hILperp}[1]{h_{1L}^{\perp #1}}
\newcommand{\hIperp}[1]{h_1^{\perp #1}}
\newcommand{\DI}[1]{D_1^{#1}}
\newcommand{\DITperp}[1]{D_{T}^{\perp #1}}
\newcommand{\HIperp}[1]{H_1^{\perp #1}}

\let\fITp\fITperp
\let\hIp\hIperp
\let\hILp\hILperp
\let\hITp\hITperp

\newcommand{\phiGM}[1]{\Phi_{#1}^{[\Gamma]}}
\newcommand{\phiLGM}{\Phi^{[\Gamma]}_{\Lambda^{\prime}\Lambda}}
\newcommand{\phiSGM}{\Phi^{[\Gamma]}(S)}
\newcommand{\phiAGGM}{\Phi^{[\Gamma]}(\theta,\varphi)}

\newcommand{\phip}[1]{\Phi_{#1}^{[\gamma^{+}]}}
\newcommand{\phiLp}{\Phi^{[\gamma^{+}]}_{\Lambda^{\prime}\Lambda}}
\newcommand{\phiSp}{\Phi^{[\gamma^{+}]}(S)}
\newcommand{\phiAGp}{\Phi^{[\gamma^{+}]}(\theta,\varphi)}

\newcommand{\phipV}[1]{\Phi_{#1}^{[\gamma^{+}\gamma^{5}]}}
\newcommand{\phiLpV}{\Phi^{[\gamma^{+}\gamma^{5}]}_{\Lambda^{\prime}\Lambda}}
\newcommand{\phiSpV}{\Phi^{[\gamma^{+}\gamma^{5}]}(S)}
\newcommand{\phiAGpV}{\Phi^{[\gamma^{+}\gamma^{5}]}(\theta,\varphi)}

\newcommand{\phijV}[2]{\Phi_{#2}^{[i\sigma^{#1}\gamma^{5}]}}
\newcommand{\phiLjV}[1]{\Phi^{[i\sigma^{#1}\gamma^{5}]}_{\Lambda^{\prime}\Lambda}}
\newcommand{\phiSjV}[1]{\Phi^{[i\sigma^{#1}\gamma^{5}]}(S)}
\newcommand{\phiAGjV}[1]{\Phi^{[i\sigma^{#1}\gamma^{5}]}(\theta,\varphi)}


